Robust data assimilation using $L_1$ and Huber norms

Data assimilation is the process to fuse information from priors, observations of nature, and numerical models, in order to obtain best estimates of the parameters or state of a physical system of interest. Presence of large errors in some observational data, e.g., data collected from a faulty instrument, negatively affect the quality of the overall assimilation results. This work develops a systematic framework for robust data assimilation. The new algorithms continue to produce good analyses in the presence of observation outliers. The approach is based on replacing the traditional $\L_2$ norm formulation of data assimilation problems with formulations based on $\L_1$ and Huber norms. Numerical experiments using the Lorenz-96 and the shallow water on the sphere models illustrate how the new algorithms outperform traditional data assimilation approaches in the presence of data outliers.

==> Algorithm_3DVar_HQ.tex <==
The computational procedure  is summarized in Algorithm \ref{alg:LH3DVar}.\textcolor{red}{Needs to be reformulated}
%
\begin{algorithm}
\caption{Minimize\_LH3DVar}\label{alg:LH3DVar}
\begin{algorithmic}[1]
\Procedure{Minimize\_LH3DVar}{}
\State \textbf{Input:} $\lbrack \x_i^{\rm b};\,\x_i^{\rm\{ k-1};\,\u^{\rm\{ k-1};\,\y_i;\, \mathbf{B}_i;\,\R_i; \,\mathcal{H};\, \tau \rbrack$ \Comment{\parbox[t]{.25\linewidth}{\small{$\x_i^{\rm \{k-1}$ and $\u^{\rm \{\rm k-1}$ are the current iterates of the analysis and its deviation from the mean respectively.}}}
\State \textbf{Output:} $\lbrack \x_i^{\rm \{k};\,\u^{\rm \{k} \rbrack$ 
\State Set $\mathbf{t} = \R_i^{-1/2}\, [ \HH_i\, \x_i^{\rm \{k-1} - \y_i ]\,$ \Comment{\parbox[t]{.25\linewidth}{\small{Compute the component-wise deviation from the mean}}}
\If{$\lvert\mathbf{t}_i \rvert < \tau$}\State{$\u^{\rm \{k}_i = 1$}
\Else\State{$\u^{\rm \{k}_i = \tau/\lvert \mathbf{t}_i\rvert$}
\EndIf
\State Set $\widetilde{\R}_i^{-1} = \R_i^{-1/2}\, {\rm diag} \left( \u^{\{k\}}/2 \right) \,\R_i^{-1/2}$ \Comment{\parbox[t]{.25\linewidth}{\small{Adjust the error covariances}}}
\State Solve for $\x_i^{\{\rm k}$: \[
\left[\B_i^{-1} +
\HH_i^T \widetilde{\R}_i^{-1} \HH_i \right] \, \x_i =
\B_i^{-1} \x_i^{\rm b} +
\HH_i^T\, \widetilde{\R}_i^{-1}  \y_i.
\]
\EndProcedure
\end{algorithmic}
\end{algorithm}
%


==> Algorithm_3DVar_Huber.tex <==
%
The overall computational procedure is summarized in Algorithm \ref{alg:LHS3DVar}. \textcolor{red}{Needs rewriting.}
%%
\begin{algorithm}
\caption{Minimize3DVar\_HuberShrinkage}\label{alg:LHS3DVar}
\begin{algorithmic}[1]
\Procedure{Minimize3DVar\_HuberShrinkage}{}
\State \textbf{Input:} $\lbrack \x_i^{\rm b};\,\x_i^{\rm g};\,\y_i;\, \mathbf{B}_i;\,\R_i; \,\mathcal{H};\,\bm{\lambda}^{\rm g};\,\mu;\, \text{\scriptsize{TOL}};\,\tau \rbrack$ \Comment{\parbox[t]{.25\linewidth}{\small{$\x_i^{\rm g}$ and $\bm{\lambda}_i^{\rm g}$ are initial guesses}}}
\State \textbf{Output:} $\lbrack \x_i^{\rm a} \rbrack$ 
\State Set $\z_i = \R_i^{-1/2}\, [ \HH_i\, \x_i^{\rm g} - \y_i ]\,$ \Comment{\parbox[t]{.25\linewidth}{\small{Fix $\z_i$}}}
\State Set $\mathbf{b}_{\rm RHS} = \B_i^{-1} \x_i^{\rm b} + \HH_i^T\, \R_i^{-1/2}\, \left[ \R_i^{-1/2} \y_i + \mu\, \z_i - \bm{\lambda} \right]$
\State Set $A_{\rm LHS} = \left[\B_i^{-1} + \mu \,\HH_i^T \R_i^{-1} \HH_i \right]$
\State Solve $A_{\rm LHS} \x_i^{\rm new} = \mathbf{b}_{\rm RHS}$
\Comment{\parbox[t]{.25\linewidth}{\small{Solve the linear system for $\x_i^{\rm new}$}}}
\State Set $d = \R_i^{-1/2} \, [\mathcal{H}(\x^{\rm new}_i) -\y_i]$
\If{$\lvert d_i\rvert > \tau$}\State{$\z_i = \displaystyle\max \left \{ \| d_i - \bm{\lambda} / \mu \|_2 - \frac{1}{\mu}, 0 \right \} \cdot
\frac{ d_i - \bm{\lambda} / \mu }
{ \| d_i - \bm{\lambda} / \mu \|_2 }.$}
\Else\State{$\z_i = \displaystyle\frac{\mu}{1+ \mu} ( d_i - \bm{\lambda} / \mu )$}
\EndIf
\State Update $\bm{\lambda} := \bm{\lambda} - \R_i^{-1/2} \, [ \mathcal{H}(\x^{\rm new}_i) - \y_i ] + \z_i.$
 \If{$\|\z_i - \R_i^{-1/2} \, [ \mathcal{H}(\x^{\rm new}_i) - \y_i ]\| < \text{\scriptsize{TOL}}$} \State{$\x_i^{\rm a} = \x_i^{\rm new}$} 
  \Else\State {$\x_i^{\rm g} = \x_i^{\rm new}$, goto step 4.}
  \State{$\mu =\mu\times {\rm fac}$}
  \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%


==> Algorithm_3DVar_L1.tex <==
The steps to be followed for a linear observation operator are explained systematically in Algorithm \ref{alg:L13DVar}.
%\textcolor{red}{Rewrite Algorithm \ref{alg:L13DVar} for the nonlinear problem and using the new notation.}
%%
% \begin{algorithm}
%\caption{L1-3D-Var}\label{alg:L13DVar}
%\begin{algorithmic}[1]
%\Procedure{Minimize\_L13DVar}{}
%\State \textbf{Input:} $\lbrack \x_i^{\rm b};\,\x_i^{\rm g};\,\y_i;\, \mathbf{B}_i;\,\R_i; \,\mathcal{H};\,\bm{\lambda}^{\rm g};\,\mu;\, \text{\scriptsize{TOL}} \rbrack$ \Comment{\parbox[t]{.25\linewidth}{\small{$\x_i^{\rm g}$ and $\bm{\lambda}_i^{\rm g}$ are initial guesses}}}
%\State \textbf{Output:} $\lbrack \x_i^{\rm a} \rbrack$ 
%\State Set $\z_i = \R_i^{-1/2}\, [ \HH_i\, \x_i^{\rm g} - \y_i ]\,$ \Comment{\parbox[t]{.25\linewidth}{\small{Fix $\z_i$}}}
%\State Set $\mathbf{b}_{\rm RHS} = \B_i^{-1} \x_i^{\rm b} + \HH_i^T\, \R_i^{-1/2}\, \left[ \R_i^{-1/2} \y_i + \mu\, \z_i - \bm{\lambda} \right]$
%\State Set $A_{\rm LHS} = \left[\B_i^{-1} + \mu \,\HH_i^T \R_i^{-1} \HH_i \right]$
%\State Solve $A_{\rm LHS} \x_i^{\rm new} = \mathbf{b}_{\rm RHS}$
%\Comment{\parbox[t]{.25\linewidth}{\small{Solve the linear system for $\x_i^{\rm new}$}}}
%\State Set $d_i = \R_i^{-1/2} \, [\mathcal{H}(\x^{\rm new}_i) -\y_i]$
%\State Evaluate $\z_i = \displaystyle\max \left \{ \| d_i - \bm{\lambda} / \mu \|_2 - \frac{1}{\mu}, 0 \right \} \cdot
%\frac{ d_i - \bm{\lambda} / \mu }
%{ \| d_i - \bm{\lambda} / \mu \|_2 }.$
%\State Update $\bm{\lambda} := \bm{\lambda} - \R_i^{-1/2} \, [ \mathcal{H}(\x^{\rm new}_i) - \y_i ] + \z_i.$
% \If{$\|\z_i - \R_i^{-1/2} \, [ \mathcal{H}(\x^{\rm new}_i) - \y_i ]\| < \text{\scriptsize{TOL}}$} \State{$\x_i^{\rm a} = \x_i^{\rm new}$} 
%  \Else\State {$\x_i^{\rm g} = \x_i^{\rm new}$, goto step 4.}
%  \State{$\mu =\mu\times {\rm fac}$}
%  \EndIf
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%%
%
% % %
% For a given number of maximum iterations, {\scriptsize{ITR}}, and a tolerance {\scriptsize{TOL}} the computational procedure for time $i$ is summarized in Algorithm \ref{alg:L13DVarb}.
 % %
  \begin{algorithm}
  \caption{L1-3D-Var}\label{alg:L13DVar}
  \begin{algorithmic}[1]
  \Procedure{Minimize\_L13DVar}{}
 \State \textbf{Input:} $\lbrack \x_i^{\rm b};\,\x_i^{\{0\}};\,\y_i;\, \mathbf{B}_i;\,\R_i; \,\mathbf{H}_i;\,\bm{\lambda}^{\{0\}};\,\mu;\, \text{\scriptsize{TOL}};\,\text{\scriptsize{ITR}}  \rbrack$ \Comment{\parbox[t]{.25\linewidth}{\small{$\x_i^{\{0\}}$ and $\bm{\lambda}_i^{\{0\}}$ are initial guesses}}}
  \State \textbf{Output:} $\lbrack \x_i^{\rm a} \rbrack$ 
  \State Initialize $\z_i^{\{0\}} = \R_i^{-1/2}\, [ \HH_i\, \x_i^{\{0\}} - \y_i ]\,$ 
  \For $\quad k=0,1,\dots,\text{\scriptsize{ITR}} $
  \State Solve for $\x_i^{\{k+1\}}$ by following the procedure in equation \eqref{eqn:L1_modified_3dvar}.
  \State Set $\displaystyle\mathbf{d}_i^{\{k+1\}}$ using the expression in \eqref{eqn:increment}
  \State Evaluate $\z^{\{k+1\}}_i$ using equation \eqref{eqn:shrinkage-L1}.
  \State Update $\bm{\lambda}_i^{\{k+1\}} := \bm{\lambda}_i^{\{k\}} - \mathbf{d}^{\{k+1\}}_i + \z^{\{k+1\}}_i.$
   \If{$\|\bm{\lambda}_i^{\{k+1\}} - \bm{\lambda}_i^{\{k\}}\| < \text{\scriptsize{TOL}}$} \State{$\x_i^{\rm a} = \x_i^{\{k+1\}}$} , \bf{STOP}
   \Else
    \State{$\mu :=\mu\times \rho\,, \rho > 1$}
    \EndIf
  \EndFor
  \EndProcedure
  \end{algorithmic}
  \end{algorithm}
 % %
 % 

